Aging with GRACE: Lifelong Model Editing with Discrete Key-Value Adaptors

Deployed language models decay over time due to shifting inputs, changing user needs, or emergent world-knowledge gaps. When such problems are identified, we want to make targeted edits while avoiding expensive retraining. However, current model editors, which modify such behaviors of pre-trained models, degrade model performance quickly across multiple, sequential edits. We propose GRACE, a lifelong model editing method, which implements spot-fixes on streaming errors of a deployed model, ensuring minimal impact on unrelated inputs. GRACE writes new mappings into a pre-trained model's latent space, creating a discrete, local codebook of edits without altering model weights. This is the first method enabling thousands of sequential edits using only streaming errors. Our experiments on T5, BERT, and GPT models show GRACE's state-of-the-art performance in making and retaining edits, while generalizing to unseen inputs. Our code is available at https://www.github.com/thartvigsen/grace}.

==> tables/main_results_no_citations.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{3.7pt}     % slight adjustment to fit text width
\setlength{\cmidrulekern}{0.25em}
\resizebox{\linewidth}{!}{
\begin{tabular}{l*{13}{c}}
\toprule
 & \multicolumn{4}{c}{\textbf{zsRE} (T5; F1 $\uparrow$)} & \multicolumn{4}{c}{\textbf{SCOTUS} (BERT; Acc $\uparrow$)}  & \multicolumn{5}{c}{\textbf{Hallucination} (GPT2-XL; PPL $\downarrow$)} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-14}
\textbf{Method} & TRR & ERR & \textit{Avg.} & \textit{\#E} & TRR & ERR & \textit{Avg.} & \textit{\#E} & TRR & ERR & ARR & \textit{\#E} & time (m)\\
\midrule
FT              & .56 & .82 & \textit{.69} & 1000 & .52 & .52 & \textit{.52} & 415 & 1449.3 & 28.14 & 107.76 & 1392 & .26 (.07)\\
FT+EWC & .51 & .82 & \textit{.66} & 1000 & .67 & .50 & \textit{.58} & 408 & 1485.7 & 29.24 & 109.59 & 1392 & .29 (.06)\\
FT+Retrain & .27 & .99 & \textit{.63} & 1000 & .67 & \textbf{.83} & \textit{.75} & 403 & 2394.3 & 35.34 & 195.82 & 1392 & 23.4 (13.2)\\
MEND            & .25 & .27 & \textit{.26} & 1000 & .19 & .27 & \textit{.23} & 672 & 1369.8 & 1754.9 & 2902.5 & 1392 & .63 (.10) \\
Defer          & \textbf{.72} & .31 & \textit{.52} & 1000 & .33 & .41 & \textit{.37} & 506 & 8183.7 & 133.3 & 10.04 & 1392 & .07 (.02) \\
ROME            & --- & --- & --- & --- & --- & --- & --- & --- & 30.28 & 103.82 & 14.02 & 1392 & \ .64 (.28)\\
Memory                                  & .25 & .27 & \textit{.26} & 1000 & .21 & .20 & \textit{.21} & 780 & 25.47 & 79.30 & 10.07 & 1392 & .11 (.02) \\
% \midrule
\cdashlinelr{1-14}
\multirow{2.25}{*}{\method} & .69 & \textbf{.96} & \textbf{\textit{.82}} & 1000 & \textbf{.81} & .82 & \textbf{\textit{.82}} & 381 & \textbf{15.84} & \textbf{7.14} & \textbf{10.00} & 1392 & .13 (.02) \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-14}
& \multicolumn{4}{c}{\textit{137 keys (7.30 edits/key)}} & \multicolumn{4}{c}{\textit{252 keys (1.51 edits/key)}} & \multicolumn{5}{c}{\textit{1341 keys (1.04 edits/key)}}\\
\bottomrule\\
\end{tabular}
}
\caption{Comparison of \method to existing methods. Parentheses in \textit{time} denote standard deviation. We add the number of keys that \method used and compute time in minutes. GRACE achieves the best TRR/ERR balance while making edits faster than the comparisons and using small codebooks for zsRE and SCOTUS. A large codebook is expected for Hallucination, since each edit label is unique.}
\end{table}
